3-Majority and 2-Choices with Many Opinions

We present the first nearly-optimal bounds on the consensus time for the well-known synchronous consensus dynamics, specifically 3-Majority and 2-Choices, for an arbitrary number of opinions. In synchronous consensus dynamics, we consider an $n$-vertex complete graph with self-loops, where each vertex holds an opinion from $\{1,\dots,k\}$. At each discrete-time round, all vertices update their opinions simultaneously according to a given protocol. The goal is to reach a consensus, where all vertices support the same opinion. In 3-Majority, each vertex chooses three random neighbors with replacement and updates its opinion to match the majority, with ties broken randomly. In 2-Choices, each vertex chooses two random neighbors with replacement. If the selected vertices hold the same opinion, the vertex adopts that opinion. Otherwise, it retains its current opinion for that round. Improving upon a line of work [Becchetti et al., SPAA'14], [Becchetti et al., SODA'16], [Berenbrink et al., PODC'17], [Ghaffari and Lengler, PODC'18], we prove that, for every $2\le k \le n$, 3-Majority (resp.\ 2-Choices) reaches consensus within $\widetilde{\Theta}(\min\{k,\sqrt{n}\})$ (resp.\ $\widetilde{\Theta}(k)$) rounds with high probability. Prior to this work, the best known upper bound on the consensus time of 3-Majority was $\widetilde{O}(k)$ if $k \ll n^{1/3}$ and $\widetilde{O}(n^{2/3})$ otherwise, and for 2-Choices, the consensus time was known to be $\widetilde{O}(k)$ for $k\ll \sqrt{n}$.

==> many_opinions.tex <==
\subsection{Dynamics with Many Opinions}
In this section, we show that the $ \ell^2 $-norm $ \alphanorm_t $ reaches $ \sqrt{\log n/n} $ within $ O(\log n/\alphanorm_0) $ rounds with high probability in the synchronous 3-Majority.
We also deal with the other models.
%
\begin{lemma}[Growth of $ \alphanorm_t $] \label{lem:taunormplus}
  Consider one of the synchronous 3-Majority, synchronous 2-Choices, or asynchronous 3-Majority.
  Let $C>\mathrm{e}^{-1}$ and $\epsilon\in(0,1)$ be arbitrary positive constants and suppose $\frac{C^2\lg^2n}{n}\leq \xnorm\leq 1-\varepsilon$.
  Then,
  \begin{align*} 
     \Pr\qty[ \taunormplus \ge T ] \le 
     \begin{cases}
      \frac{64\e^2}{\epsilon}\cdot  \frac{\xnorm n}{T}	& \text{for 3-Majority},\\
      \frac{192\e^2}{\epsilon^2}\cdot  \frac{\xnorm n^2}{T}	& \text{for 2-Choices}.
     \end{cases}
  \end{align*}
  %where $ \tauivanish,\taunormdown,\tauiactive $ are defined in \cref{def:tauivanish,def:taunormup,def:taualpha}.
\end{lemma}



\begin{proof}[Proof of \cref{thm:main theorem}]
  Consider the synchronous 3-Majority and let $C>0$ be a sufficiently large constant.
  From \cref{lem:taunormplus} for $\xnorm = C\sqrt{\log n/n}$, we have $\alphanorm_t \ge C\sqrt{\log n/n}$ with probability $1/2$ within $t=O(\sqrt{n\log n})$ rounds.
  Repeating this argument for $O(\log n)$ times,
  with high probability, we have $\alphanorm_T \ge C\sqrt{\log n/n}$ for some $T=O(\sqrt{n}(\log n)^{1.5})$.


  Suppose that the initial configuration satisfies $ \alphanorm_0 \ge  C\sqrt{n\log n}$.
  Fix any two distinct opinions $ i,j $.
  From \cref{lem:tauweak}, either $ i $ or $ j $ becomes weak within $ O(\log n/\alphanorm_0)$ rounds with probability $ 1-O(n^{-10}) $.
  Moreover, every weak opinion vanishes within additional $ O(\log n/\alphanorm_0) $ rounds from \cref{lem:weakvanish} with probability $ 1-O(n^{-10}) $.
  Therefore, by the union bound over $ i\ne j $, with probability $ 1-O(n^{-8}) $,
    for any pair of distinct opinions, either $ i $ or $ j $ vanishes within $ O(\log n/\alphanorm_0) $ rounds.
  This indicates that the configuration achieves consensus.

  We prove the claim of plurality consensus.
  If the most popular opinion $i\in[k]$ satisfies $\alpha_i - \alpha_j \ge C\sqrt{\log n/n}$ for all $j\ne i$, then
  from the “Furthermore" part of \cref{lem:tauweak} (combined with the union bound over $j\ne i$),
  the opinion $i$ never become weak during the process.
  This implies that the process consensus with the opinion $i$ with high probability.

  The proof for 2-Choices can be obtained by the same way.
\end{proof}

